Exploring Cosmic Origins with CORE: Inflation

We forecast the scientific capabilities to improve our understanding of cosmic inflation of CORE, a proposed CMB space satellite submitted in response to the ESA fifth call for a medium-size mission opportunity. The CORE satellite will map the CMB anisotropies in temperature and polarization in 19 frequency channels spanning the range 60-600 GHz. CORE will have an aggregate noise sensitivity of $1.7 \mu$K$\cdot \,$arcmin and an angular resolution of 5' at 200 GHz. We explore the impact of telescope size and noise sensitivity on the inflation science return by making forecasts for several instrumental configurations. This study assumes that the lower and higher frequency channels suffice to remove foreground contaminations and complements other related studies of component separation and systematic effects, which will be reported in other papers of the series "Exploring Cosmic Origins with CORE." We forecast the capability to determine key inflationary parameters, to lower the detection limit for the tensor-to-scalar ratio down to the $10^{-3}$ level, to chart the landscape of single field slow-roll inflationary models, to constrain the epoch of reheating, thus connecting inflation to the standard radiation-matter dominated Big Bang era, to reconstruct the primordial power spectrum, to constrain the contribution from isocurvature perturbations to the $10^{-3}$ level, to improve constraints on the cosmic string tension to a level below the presumptive GUT scale, and to improve the current measurements of primordial non-Gaussianities down to the $f_{NL}^{\rm local} < 1$ level. For all the models explored, CORE alone will improve significantly on the present constraints on the physics of inflation. Its capabilities will be further enhanced by combining with complementary future cosmological observations.

==> section_six/Section_features_2_old.tex <==
The fundamental contact of inflationary theory with observation comes via a model's prediction of the primordial scalar \(\mathcal{P}_\mathcal{R}\) and tensor \(\mathcal{P}_\mathcal{T}\) power spectra. These are processed by cosmological transfer functions into predictions of CMB temperature and polarization multipoles \(C_\ell\). Comparing the theoretical \(C_\ell\)'s with the observed values yields constraints on the inflationary model parameters.

In this section we reverse this procedure, and reconstruct the primordial power spectra directly from the data. This has been successfully performed on \Planck\ 2015 data~\cite{Ade:2015lrj} for the scalar primordial power spectrum using the methods of Gauthier \& Bucher~\cite{Gauthier2012}, Vazquez et.~al.~\cite{Vazquez2012}, Aslanyan et.~al.~\cite{Aslanyan2014} and the methods of Bond et.~al.\ described in~\cite{Ade:2015lrj}.


\subsection{Primordial power spectra reconstruction methodology}
\begin{figure}[tp]
    \centering
    \begin{tikzpicture}

        \newcommand{\movablecross}[2]{%
            \draw[->](#1) -- ++(0:#2);
            \draw[->](#1) -- ++(90:#2);
            \draw[->](#1) -- ++(180:#2);
            \draw[->](#1) -- ++(270:#2);
            \fill[red!70!black] (#1) circle (2pt);
        }

        \newcommand{\movablevert}[2]{%
            \draw[->](#1) -- ++(90:#2);
            \draw[->](#1) -- ++(270:#2);
            \fill[red!70!black] (#1) circle (2pt);
        }


    % Axes
        \draw [<->,thick] (6,0) coordinate (X) -- (0,0) coordinate (O) -- (0,4) coordinate (Y);

    % Axes labels
        \draw (X) node[right]  {\(\log k [ \mathrm{Mpc}^{-1}]\)}; 
        \draw (Y) node[above] {\(\log(10^{10}\PPS)\)};

    % Reconstruction line
        \draw (0.5,1.5) coordinate (A) -- (1.75,2.25) coordinate (B) -- (3,1.5) coordinate (C) -- (5,2.5) coordinate(D);

    % Crosses
        \movablevert{A}{0.4}
        \movablecross{B}{0.4}
        \movablecross{C}{0.4}
        \movablevert{D}{0.4}

    % Node labels
        \draw (A) node[below right] {\((k_1,\PPS_{1})\)};
        \draw (B) node[above right] {\((k_2,\PPS_{2})\)};
        \draw (C) node[below right] {\((k_3,\PPS_{3})\)};
        \draw (D) node[above left] {\((k_{\Nknots},\PPS_{\Nknots})\)};

    % Draw prior widths
        \coordinate(A1) at ($(O)!(A)!(X)$);
        \coordinate(D1) at ($(O)!(D)!(X)$);
        \draw (A1) node[below] {$10^{-4}$};
        \draw (D1) node[below] {$10^{-0.3}$};

        \coordinate(ymin) at (O |-0,0.75);
        \coordinate(ymax) at (O |-0,3.5);

        \draw[-,dashed] (ymin) -- (X |- ymin);
        \draw[-,dashed] (ymax) -- (X |- ymax);
        \draw[-,dashed] (A1) -- (A1 |- Y);
        \draw[-,dashed] (D1) -- (D1 |- Y);

        \draw (ymin) node[left] {2};
        \draw (ymax) node[left] {4};

% put some ellipses in between the start and end point

    \end{tikzpicture}
    \caption{%
    The scalar primordial power spectra are reconstructed using \(\Nknots\)-point interpolating logarithmic splines. The positions of the points in the \((k,\PPS)\) plane are treated as likelihood parameters with log-uniform priors. Further, the \(k\)-positions sorted {\em a-priori\/} such that \({k_1<k_2<\cdots<k_{\Nknots}}\) with \(k_1\) and \(k_\Nknots\) fixed. Units of \(k\) are inverse megaparsecs.}\label{fig:linear_spline_reconstruction}
\end{figure}

To reconstruct primordial power spectra, we follow the methodology of Section~8.2 of the \Planck\ inflation paper~\cite{Ade:2015lrj}. Instead of using the traditional amplitude-tilt parameterization (\(A_\mathrm{s},n_\mathrm{s}\)), we instead use an \(\Nknots\)-point interpolating logarithmic spline (Figure~\ref{fig:linear_spline_reconstruction}), with the positions of the knots considered as free parameters in the full posterior distribution. 

We compute posteriors (conditioned on \(\Nknots\)) using the PolyChord nested sampler~\cite{Handley2015a,Handley2015b}, also varying the cosmological and any nuisance parameters. We then use evidence values for each model to correctly marginalize out the number of knots \(\Nknots\).

To plot our reconstructions of the power spectra, we compute the marginalized posterior distribution of \(\log\PPS\) conditioned on \(k\). The iso-probability confidence intervals are then plotted in the \(k,\PPS\) plane (e.g.\ Figure~\ref{fig:PPSR}).

To quantify the constraining power of a given experiment, we use the conditional Kullback-Leibler (KL) divergence~\cite{Hee2016}, defined in equation~\ref{eq:DKL}. For our reconstructions, we compute the KL divergence of each distribution conditioned on \(k\) and \(\Nknots\), and then marginalize over \(\Nknots\) using evidences to produce a \(k\)-dependent number which quantifies the logarithmic compression (i.e.\ information) that each experiment provides at each value of \(k\) (e.g.\ Figure~\ref{fig:DKLPPSR}).

This reconstruction approach has the advantage of being somewhat agnostic to any specific inflation model, and constitutes a ``blind'' reconstruction of the power spectra. One could of course also search for parameterized features, as is discussed in Section~9 of the \Planck\ inflation paper~\cite{Ade:2015lrj}, but for the purposes of forecasting this produces a somewhat self-fulfilling set of reconstructions. In this section we shall therefore focus on answering the question as to how well a blind reconstruction could pick up a variety of features using CORE-M5 data resolution. This approach is by no means unique. Other authors have used a binned spectrum~\cite{Hazra:2013pps}, cubic splines~\cite{CubicSplines} and cross-validation~\cite{RedStraightNoBends}, as well as reconstructions motivated by phenomenology~\cite{PhenomenologicalPPS} or inflationary-models~\cite{Hazra:2016pps,Hazra:2014pps}. The approach chosen for this section is motivated more by its conceptual simplicity than anything else.


\subsection{Featureless scalar power spectrum}

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth ]{section_six/figures/posterior_featureless_2.jpg}
    \includegraphics[width=0.45\textwidth ]{section_six/figures/posterior_featureless_zoom_2.jpg}
    \caption{Left: Reconstruction of a simulated featureless scalar power spectrum, for a CORE-M5 experiment (in red), 
in comparison with existing constraints provided by \Planck\ (in blue). Right: Zoomed-in version of the left figure to show 
the order of magnitude increase in constraining power that would be provided by CORE.}\label{fig:PPSR}
\end{figure}

\begin{figure}
    \centering
    \includegraphics{section_six/figures/DKL_2.pdf}
    \caption{The amount of information that CORE experiments would provide on the scalar primordial power spectrum. 
The Kullback-Leibler divergence shows that all configurations of the experiment provide a similar level 
of information. This is at a level an order of magnitude more information than \Planck\ 2015 provides, and a log unit more than \Planck's theoretical constraint. As expected, the prior-to-posterior compression 
drops off at low-$\ell$ due to cosmic variance, and high-$\ell$ at the limits of the experiment.}\label{fig:DKLPPSR}
\end{figure}

To quantify the basic constraining power of the experiments detailed in 
Tables~\ref{tab:CORE-bands} and~\ref{tab:specifications}, we begin by examining 
how well these experiments could constrain a featureless scalar power spectrum. Simulated likelihoods are 
generated from a featureless tilted power spectrum with $n_\mathrm{s}=0.96$ and $A_\mathrm{s}=2.1\times10^{-9}$ 
with \(TT\),\(TE\) \& \(EE\) data for COrE+, LiteCORE-120, LiteCORE-80, LiteBIRD and CORE-M5 experiments. 
\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth ]{section_six/figures/posterior_wiggly_2.jpg}
    \includegraphics[width=0.45\textwidth ]{section_six/figures/posterior_cs_2.pdf}
\caption{As in Figure~\protect\ref{fig:PPSR}, but now reconstructing a simulated power spectrum with features (black lines). 
Left: Cut-off as would be generated by a brief period of fast-roll expansion prior to slow roll inflation. The additional 
constraining power provided by CORE would allow detection of low-$\ell$ features such as cutoffs and wiggles. 
Right: Reconstruction of higher-$\ell$ linearly-sinusoidal wiggles
generated by a reduction in the speed of sound of the inflaton, as
described in Section 2.3.3. In this last case, the
reconstruction only picks up the feature when the prior on the nodes' positions is restricted to the region where the feature is active; the
smaller-scale wiggles prove to be harder to reconstruct.}
\label{fig:PPSR_wiggles}
\end{figure}
\afterpage{%
\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{section_six/figures/posterior_monodromy_2.jpg}
    \includegraphics[width=0.45\textwidth]{section_six/figures/ballardini_wiggles_2.pdf}
    \caption{Left: As in Figure~\protect\ref{fig:PPSR}, but now reconstructing a 
simulated power spectrum with 
low frequency sinusoidal logarithmic oscillations (black line), with $A_{\log}=0.03, \omega_{\log}=3$
and $\psi_{\log}=0$. Right: constraints on superimposed sinusoidal logarithmic oscillations with an higher frequency, comparable 
to those providing a best-fit to \Planck\ 2015 data \cite{Ade:2015lrj}.
Whereas a blind reconstruction technique is unsuitable for high 
frequency oscillations, CORE-M5 performs better than LiteBIRD or \Planck\ in combination with Euclid spectroscopic galaxy clustering for this type of parameterized features.
Contours indicate 68\% confidence intervals.}\label{fig:PPSR_monodromy}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=0.79\textwidth]{section_six/figures/COrEp_tensors_featureless_2.pdf}
    \caption{Simultaneous reconstructions of the tensor (lower, green) and scalar (upper, red) power spectra for CORE-M5 forecast if \(r=0.001\).\label{fig:marg_COrE}}
\end{figure}}

Figure~\ref{fig:PPSR} shows the marginalized posterior distribution for the CORE-M5 experiment. 
As usual, the reconstructions demonstrate the lack of reconstructive power at low-$k$ due to 
cosmic variance, and the inability to reconstruct above the resolving power of $\ell\sim3000$. 
CORE-M5 provides an order of magnitude better constraint on the amplitude of the power spectrum relative to \Planck\ 2015 data (shown for reference in blue).



To quantify the level of this increase in information, Figure~\ref{fig:DKLPPSR} shows the information 
gain for each of these experiments at each value of \(k\) in comparison with \Planck. One can see that 
all three configurations provide similar levels of information on the primordial power spectrum, and an 
order of magnitude more information than \Planck, with LiteBIRD and LiteCORE-80 failing to provide information above $\ell\sim1350$ and $2400$ respectively.

\subsection{Scalar power spectrum with wiggles and cutoffs}

With such strong constraining power, any of these CORE experiments would be able to detect features in the primordial power 
spectrum that are currently unresolved using \Planck\ data. To show this, we produced a likelihood for a wiggly power spectrum 
as would be generated by an epoch of fast-roll inflation prior to slow roll~\cite{Contaldi2003}. 
The left hand plot of Figure~\ref{fig:PPSR_wiggles} shows that CORE-M5 has the capacity to blindly 
reconstruct a cutoff and the first oscillation which could be hidden beneath \Planck\ 2015 resolution.

CORE experiments would also be capable of reconstructing smaller localized features, 
such as those produced by reduced adiabatic sound speeds (Section~\protect\ref{sssec:features}), as demonstrated in Figure~\ref{fig:PPSR_wiggles}. 


\subsection{Superimposed logarithmic oscillations}

Resonant models including periodic oscillations in the potential lead to superimposed sinusoidal oscillation in the spectrum and bispectrum
\cite{Chen:2008wn}, as discussed in Section 2.
The periodic oscillations appearing in axion monodromy \cite{Silverstein:2008sg,McAllister:2008hb} belong to this general class of models \cite{Flauger:2009ab}.
We consider the following phenomenological parameterization:
\begin{equation}
    \mathcal{P}_\mathcal{R}(k) = A_\mathrm{s} {\left( \frac{k}{k_*} \right)}^{n_\mathrm{s} - 1} \left( 1 + A_{\log} \sin[\omega_{\log} k + \psi_{\log}] \right).
\label{resonant}
\end{equation}
As is shown in Figure~\ref{fig:PPSR_monodromy}, CORE-M5 also has the resolving power to blindly reconstruct logarithmic oscillations with an amplitude at a percent level 
for low frequencies, i.e. $\omega_{\log} = 3$. For higher frequencies, the blind reconstruction scheme would require prohibitively large numbers of knots.
Nevertheless, as is shown in the right-hand panel of Figure~\ref{fig:PPSR_monodromy}, CORE-M5 is still capable of extracting information
about such models, by directly constraining the parameters of the superimposed oscillations in Eq. (\ref{resonant}). 
Further detail on the Fisher forecast methodology for this approach is provided by~\cite{Ballardini2016}.

\subsection{Reconstructing the tensor power spectrum}

Finally, we demonstrate that if there is a detectable scalar-to-tensor ratio, 
then CORE-M5 would also be able to reconstruct this spectrum. Figure~\ref{fig:marg_COrE} 
shows a simultaneous reconstruction of both the scalar and tensor power spectrum, 
where we use two independent reconstructions on simulated data with a flat tensor power spectrum for \(r=0.001\).


==> section_three/tables/section_three.tex <==
%In this section we concisely present the methodology used for our forecasts 
%based on the cosmological information contained in the temperature, polarization and lensing power spectra. We then present 
%the expected unsertainties on the key inflationary parameters.

%In this section we investigate the expected constraints for the physics of inflation of the ESA M5 mission \coremfive\ in 
%M5 CMB space mission proposed to ESA. 
%The purpose of this paper is to study the capabilities of the ESA M5 mission proposal and 
In this section we describe the methodology adopted for the forecasts in the rest of the paper.
%our assessment of the implication for the physics of inflation 
%from CORE-M5. 
%in comparison with those from other experimental configurations. 
%CMB space missions.
%, such as a LiteBIRD-ext 
%configuration \cite{Errard2016} for JAXA LiteBird \cite{2014JLTP..176..733M},
%three configurations with the same noise sensitivity per arcmin, 
%but higher angular resolution thanks to a larger telescope of 80 cm (LiteCore-80) or 120 cm (LiteCore-120) or 
%150 cm (LiteCore-150), 
%the ESA CDF LiteCore designs 
%and the CORE+ proposal submitted to the previous ESA M4 mission call.
%For all these configurations we consider a conservative choice for the frequency channels, 
%assuming that the channels at lower and higher frequencies help in mitigating the foreground contamination.  
%This comparison therefore sheds light on the role of different angular resolution and raw detector sensitivities on the implication
%for inflation which are expected from future CMB space missions.


Assuming that CMB anisotropies are Gaussian and statistically isotropic,
we use the following $\chi_\mathrm{eff}^2$ for our science forecasts \cite{Knox:1995dq,Hamimeche:2008ai}:
\be
\chi_\mathrm{eff}^2 = - 2 \ln {\cal L} = \sum_{\ell} (2\ell+1) f_\mathrm{sky} \left\{ \mathrm{Tr} [ \hat{{\bf C}}_\ell \bar{{\bf C}}_\ell^{-1}] +
\ln |\hat{{\bf C}}_\ell \bar{{\bf C}}_\ell^{-1}| - n \right\},
\end{equation}
where $\bar{{\bf C}}_\ell$ and $\hat{{\bf C}}_\ell$ denote the theoretical and observed data covariance matrices, respectively,
and $N$ is a normalization factor. The covariance matrix depends on the power spectra $C_\ell^{XY}$ where $X$ and $Y$ 
can be $\{T,E\}$ (with $n=2$), $\{T,E,B\}$ or $\{T,E,d\}$ (with $n=3$), $\{T,E,B,P\}$ (with $n=4$) where $P$ denotes lensing potential. 
In the most general case the observed covariance is
%\begin{equation}
%\label{eq:covariance_definition}
%\bar{\boldsymbol{C}}_\ell \equiv
% \begin{bmatrix}
%\bar{C}_\ell^{TT} + N_\ell^{TT} & \bar{C}_\ell^{TE} & 0 & \bar{C}_\ell^{Td} \\
%\bar{C}_\ell^{TE} & \bar{C}_\ell^{EE} + N_\ell^{EE} & 0 & \bar{C}_\ell^{Ed} \\
%0 & 0 & \bar{C}_\ell^{BB} + N_\ell^{BB} & 0  \\
%\bar{C}_\ell^{Td}  & \bar{C}_\ell^{Ed} & 0 & \bar{C}_\ell^{dd} + N_\ell^{dd}
%\end{bmatrix} ,
%\end{equation}
\begin{equation}
\label{eq:covariance_definition}
\bar{\boldsymbol{C}}_\ell \equiv
 \begin{bmatrix}
\bar{C}_\ell^{TT} + N_\ell^{TT} & \bar{C}_\ell^{TE} & 0 & \bar{C}_\ell^{TP} \\
\bar{C}_\ell^{TE} & \bar{C}_\ell^{EE} + N_\ell^{EE} & 0 & \bar{C}_\ell^{EP} \\
0 & 0 & \bar{C}_\ell^{BB} + N_\ell^{BB} & 0  \\
\bar{C}_\ell^{TP}  & \bar{C}_\ell^{EP} & 0 & \bar{C}_\ell^{PP} + N_\ell^{PP}
\end{bmatrix} ,
\end{equation}
where $N_\ell^{XY}$ are the noise power spectra.
%, which would 
This accounts %for $X = \{T,E,B\}$ 
for the instrumental noise, $N_\ell^{\mathrm XX, inst}$,
%for the effects due to imperfect foreground removal 
and for delensing when $X=B$. 
For any experimental configuration studied %considered for $X = \{T,E,B\}$,
we will consider an inverse-variance weighted sum of the noise sensitivity convolved with a Gaussian beam window function for each frequency channel $\nu$:
%over the cosmological channels listed in Table :
\be
N_\ell^{\mathrm XX, inst} = \left[ \sum_\nu \frac{1}{N_{\ell \, \nu}^{\mathrm XX, inst}} \right]^{-1} \,,
\ee
with 
\be
N_{\ell \, \nu}^{\mathrm XX, inst} = w_{X \, \nu}^{-1} \exp \left[ \ell (\ell+1) \frac{\theta_{\mathrm FWHM}}{8 \ln 2} \right]
\ee
%\ba
%N_{\ell \, \nu}^{\mathrm XX, inst} &=& w_{X \, \nu}^{-1} b_\ell^{-2} \\
%\exp \left[ \ell (\ell+1) \frac{\theta_{\mathrm FWHM}}{8 \ln 2} \right] \\
%b_\ell^2 & = & \exp \left[ - \ell (\ell+1) \frac{\theta_{\mathrm FWHM}}{8 \ln 2} \right]
%\,.
%\ea
Here $w_{{\rm E} \,, \nu}^{-1/2} = w_{{\rm B} \,, \nu}^{-1/2}$ ($=w_{{\rm T} \,,}^{-1/2} \sqrt{2})$ is the
detector noise level on a steradian patch for polarization (temperature) and % $b_\ell^2$ is the Gaussian beam window function, with
$\theta_{\rm FWHM}$ as the full width half maximum (FWHM) of the beam in radians for a given frequency channel $\nu$. 
We assume that beam and systematic uncertainties are under control 
and smaller than the statistical errors. 
%The experimental configurations are listed in of the 

%In most of this paper
Unless specified otherwise, we consider for our mock data a 
fiducial $\Lambda$CDM cosmology compatible with $Planck$ constraints \cite{planck2014-a10}. 
We assume a flat Universe with a cosmological costant, $\Omega_b h^2 = 0.02214$ and $\Omega_{c} h^2 = 0.1206$ as baryon and cold dark matter 
physical densities, respectively.
We choose the optical depth to reionization $\tau = 0.0581$, the Hubble parameter $H_0 = 66.89$ km s$^{-1}$ Mpc$^{-1}$, 
%the angular scale of the sound horizon at recombination $\theta_s = $, 
$A_{\mathrm s} = 2.1179 \times 10^{-9}$ and spectral index $n_{\mathrm s} = 0.9625$ as amplitude and tilt for the spectrum of primordial perturbations, respectively.

We use the publicly available Einstein-Boltzmann codes {\sc CAMB}\footnote{\tt
http://camb.info/}~\cite{Lewis:1999bs} or {\sc CLASS}\footnote{\tt http://class-code.net}~\cite{Lesgourgues:2011re,Blas:2011rf} to compute the 
theoretical predictions for temperature, polarization and deflection power spectra. 
We generate posterior probability
distributions for the parameters using either the Metropolis-Hastings
algorithm implemented in {\tt CosmoMC}~\mbox{\citep{Lewis:2002ah}} or
{\tt MontePython}~\mbox{\citep{Audren:2012wb}}, the nested sampling
algorithm {\tt MultiNest} \citep{Feroz:2007kg,Feroz:2008xx,Feroz:2013hea},
or {\tt PolyChord}, which combines nested sampling with slice
sampling~\citep{Handley:2015fda}. 

%we consider the following $\Lambda$CDM cosmological model compatible with $Planck$ constraints \cite{planck2014-a10}:
%\cite{PIPXLVI}:
%\be
%\{ \Omega_b h^2 = 0.0221 \,, \Omega_{\mathrm cdm} h^2 = 0.121 \,,
%h = 0.669 \,, n_{\mathrm s} = 0.9625 \,, \tau = 0.058 \,, \ln (10^{10} A_{\mathrm s}) = 3.09 \}
%\label{fiducial}
%\ee

\begin{wrapfigure}{L}{0.6\textwidth}
%\begin{figure}
%        \centering
\begin{center}
                \includegraphics[width=9cm]{section_three/figures/FGspectra_Errard2016.pdf}
\end{center}
\vspace{-1\baselineskip}
\caption{Comparison of diffuse astrophysical
foregrounds amplitudes with cosmological signals,
in particular the primordial and lensed $B$-modes.
The sensitivity to primordial signal is limited by galactic emissions and gravitational lensing (from~\cite{Errard2016}).}
\label{fig:FGspectra}
%\end{figure}
\end{wrapfigure}
 
In addition to the primary CMB temperature and polarization anisotropies, we consider the cosmological information contained in the 
CMB weak lensing - see \cite{Lewis:2006fu} for a review -, encoded in the power spectrum of the CMB lensing potential.
%the deflection field $C_\ell^{\phi phi}$.  
Most of the experimental configurations studied here allow a precise reconstruction of the CMB lensing potential.
It is known that $C_\ell^{\phi \phi}$ helps in breaking parameter degeneracies 
and help in the determination of the neutrino mass \cite{2003PhRvL..91x1301K}. We therefore fold in the CMB 
lensing information in our likelihood approach with the same methodology used in the companion paper \cite{2003PhRvL..91x1301K}.  
%and most of the experimental configurations studied here allow a precise reconstruction of the CMB lensing potential. 


%\input table_configurations.tex

CMB lensing can also be considered as a nuisance in the quest for primordial gravitational waves.
In fact, lensing mixes the $E$ and $B$ polarization modes \citep{2006PhR...429....1L}, and since
the primordial $B$-modes signal only arises from primordial tensor perturbations which are much
smaller than the scalar ones (generating $E$ polarization), lensing transfers a significant amount
of $E$ into $B$ polarization. The amplitude of these so-called lensed $B$ modes peaks around a multipole
$\ell\sim1000$ and, with $r<0.07$ at 95 \% CL \cite{2016PhRvL.116c1302B}, is always larger than the 
primordial signal on scales smaller than the reionization bump.
Lensing is therefore, after the diffuse astrophysical foregrounds, the second largest 
contaminant in the search for $r$, cf. Fig.~\ref{fig:FGspectra}.

%\newpage

%\input table_configurations.tex

Techniques have been proposed to \emph{delens} the CMB polarization maps
\citep{2015PhRvD..92d3005S,2015ApJ...807..166S,2007PhRvD..76l3009M,2004PhRvD..69d3005S,
2002PhRvL..89a1304K,2002PhRvL..89a1303K,2012JCAP...06..014S},
i.e. in order to reduce the extra \emph{variance} induced by lensing.
Delensing proposes to remove the lensing induced signal from the observed CMB, 
and that requires an estimate of the unlensed CMB as well as the matter 
distribution. The latter can be obtained either from external surveys
(cosmic shear, galaxy catalogs, 21cm, CIB) or from the CMB lensing estimate itself
(using e.g. quadratic or maximum-likelihood estimators). The former can
be obtained at first order from observed $E$-modes, since lensing is only a small correction.
Note that when delensing is performed using the internal CMB lensing
estimate, its accuracy can be improved by iterating over the delensing step, replacing the
observed CMB maps with the delensed one from a previous step.
The performance of delensing would depend on the experimental characteristics and on the choice for the matter distribution estimator
(see for a detailed analysis of the delensing efficiency and its propagation to limits on $r$ is discussed in~\cite{Errard2016}). 
In this paper we consider internal CMB delensing, in the logic to investigate the performance of each experimental configuration 
alone without the help of external data. 

The left panel of Fig.~\ref{fig:sigma_r_mnu_vs_fsky_uKarcmin_Errard2016} shows the 
delensing factor $\alpha$, introduced in~\cite{Errard2016}, as a function of the 
post-component-separation sensitivity of a CMB experiment with a Gaussian beam with 
full-width at half-maximum (FWHM) of $3'$. Plotted are three delensing methods considered in~\cite{Errard2016}: 
iterative delensing using the CMB polarization, and via cross-correlation with the cosmic infrared background (CIB) or a futuristic large scale structure survey. 
The first point to note is that delensing exploiting the correlation with futuristic large scale structures surveys only marginally surpass 
the delensing with CIB, even though the latter makes use of existing Planck data products~\cite{2015PhRvD..92d3005S}. 
Moreover, for both cross-correlation methods the sensitivity of the CMB instrument does not affect the performance in the regime $\leq 5-10\ \mu$K-arcmin, 
as the $E$-mode observations are largely cosmic-variance limited for these sensitivities. Iterative delensing using CMB polarization becomes 
more effective than the cross-correlation techniques when the post-component separation noise level is below $\sim\,3\ \mu$K-arcmin. 
Note that other quadratic combinations of CMB fields --- and, indeed, their minimum-variance combination~\cite{2002ApJ...574..566H} --- 
could outperform the ``$EBEB$'' estimator considered here in the high-noise regime.
This result is a consequence of $N_\ell^{\phi\phi}$ which continues to decrease with the instrumental sensitivity increasing, under the assumptions of 
iterative delensing~\cite{2004PhRvD..69d3005S}.
Note also that the curves become thicker as the noise level decreases: this is due to varying the observed fraction of sky between $1$ and $100\%$. 
Larger-scale experiments have access to more multipoles (assuming $\ell_{\rm min} \propto f_{\rm sky}^{-1/2}$) which can improve iterative delensing at low noise levels.
We do not show here the dependence of $\alpha$ upon the instrumental angular resolution. Yet, it is important to note 
that un-observed $E$-modes between $100 \leq \ell \leq 1000$ will significantly degrade the reconstruction of lensed $B$-modes and therefore their subtraction. 
In addition, for a given CMB map sensitivity, the reconstruction of the lensing potential will be optimized by looking 
at rather high-$\ell$ in all CMB power spectra.

%The experimental configurations studied here are listed in Table 1.
We focus on the configuration of the CMB space mission CORE-M5 recently submitted to ESA. [More details]

\input section_three/tables/table_CORE.tex


We consider a LiteBIRD-ext configuration \cite{Errard2016} 
for the JAXA LiteBIRD mission \cite{2014JLTP..176..733M} and three configurations with the
same sensitivity per arcmin, but higher angular resolution thanks 
to a larger telescope of 80 cm (LiteCore-80) or 120 cm (LiteCore-120) or 150 cm (LiteCore-150). 
%, respectively.
%We finally compare with a proposal for a CMB space mission with a 150 cm class telescope 
%to further study the impact of a better angular resolution with
%respect to the one submitted to the ESA M5 call. 
We finally compare with the COrE+ experimental configuration 
of the CMB space mission proposal previously submitted to the ESA M4 call; we denote by 
optCOrE+ its extended version with increased effective noise sensitivity due to the extension of the mission.

\input section_three/tables/table_configurations.tex

\FloatBarrier

\begin{figure}
        \centering
                \includegraphics[width=7.5cm]{section_three/figures/alpha_vs_uKarcmin_errard16.pdf}~\includegraphics[width=7.5cm]{section_three/figures/sigma_r_vs_fsky_uKarcmin_errard16.pdf}
        \caption{\textit{Left panel:} $\alpha$,
the delensing improvement, shown as a function of the noise in the CMB map after component separation.
$\alpha$ is defined as the ratio of the integrated powers between the delensed and lensed B-modes,
around the recombination bump ($20\leq\ell\leq200$). The delensing improvement is shown here using
an iterative delensing based on the observation of $E$ and $B$-modes (dark orange),
using CIB information (light orange) and using a futuristic large scale structure
survey (dark red). The result assumes FWHM=$3'$ and a multipole
range of $\sqrt{ 2\pi / f_{\rm sky}} \leq \ell \leq 3000$.
\textit{Right panel:} One-sigma limit on $r=0$, $\sigma(r=0)$,
as a function of both the noise in the CMB map and the observed
fraction of the sky. Grey (respectively black) contours correspond
to the no delensing (respectively iterative CMB delensing) case.
No foreground residuals are taken into account in this result. Figures taken from~\cite{Errard2016}. }
\label{fig:sigma_r_mnu_vs_fsky_uKarcmin_Errard2016}
\end{figure}


%\input table_configurations.tex

%\newpage


==> section_three/tables/table_CORE.tex <==
{\small
\begin{table}[h]
\begin{center}
{\footnotesize
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
Channel & FWHM  &  $N_{\rm det}$  &  $\Delta T$  &  $\Delta P$  & $\Delta I$ & $\Delta I$  & $\Delta y\times 10^6$  &  PS  ($5\sigma$) \\
GHz     &       [arcmin] &    &  [$\mu K$ arcmin] &  [$\mu K$ arcmin] &  [$\mu K_{\rm RJ}$ arcmin]  & [kJy/sr arcmin] 
&  [$y_{\rm SZ}$ arcmin] & [mJy]  \\
\hline
\hline

60      & 17.87   & 48      & 7.5          & 10.6         & 6.81          & 0.75         & -1.5         & 5.0                     \\
70      & 15.39   & 48      & 7.1          & 10           & 6.23          & 0.94         & -1.5         & 5.4              \\
80          & 13.52   & 48      & 6.8          & 9.6          & 5.76          & 1.13         & -1.5         & 5.7           \\
90         & 12.08   & 78      & 5.1          & 7.3          & 4.19          & 1.04         & -1.2         & 4.7            \\
100       & 10.92   & 78      & 5.0            & 7.1          & 3.90          & 1.2          & -1.2         & 4.9          \\
115       & 9.56    & 76      & 5.0            & 7.0            & 3.58          & 1.45         & -1.3         & 5.2         \\
130      & 8.51    & 124     & 3.9          & 5.5          & 2.55          & 1.32         & -1.2         & 4.2         \\
145      & 7.68    & 144     & 3.6          & 5.1          & 2.16          & 1.39         & -1.3         & 4.0             \\
160      & 7.01    & 144     & 3.7          & 5.2          & 1.98            & 1.55         & -1.6         & 4.1            \\
175        & 6.45    & 160     & 3.6          & 5.1          & 1.72          & 1.62         & -2.1         & 3.9         \\
195     & 5.84    & 192     & 3.5          & 4.9          & 1.41          & 1.65         & -3.8         & 3.6           \\
220      & 5.23    & 192     & 3.8          & 5.4          & 1.24          & 1.85         & -           & 3.6         \\
255      & 4.57    & 128     & 5.6          & 7.9          & 1.30          & 2.59         & 3.5          & 4.4         \\
295       & 3.99    & 128     & 7.4          & 10.5         & 1.12          & 3.01         & 2.2          & 4.5           \\
340      & 3.49    & 128     & 11.1         & 15.7         & 1.01            & 3.57         & 2.0            & 4.7             \\
390       & 3.06    & 96      & 22.0           & 31.1         & 1.08          & 5.05         & 2.8          & 5.8          \\
450      & 2.65    & 96      & 45.9         & 64.9         & 1.04            & 6.48         & 4.3          & 6.5           \\
520      & 2.29    & 96      & 116.6        & 164.8        & 1.03            & 8.56         & 8.3          & 7.4      \\
600       & 1.98    & 96      & 358.3        & 506.7        & 1.03            & 11.4         & 20.0           & 8.5            \\
\hline
\hline
Array         &              & 2100 & 1.2  & 1.7 &  &  & 0.41 &   \\
\hline
\end{tabular}
}
\end{center}
\caption{\small Proposed CORE-M5 frequency channels.
The sensitivity is calculated assuming $\Delta \nu/\nu=30\%$ bandwidth,
60\% optical efficiency, total noise of twice the expected photon noise
from the sky and the optics of the instrument at 40K temperature.
This configuration has 2100 detectors, about 45\% of which are located 
in CMB channels between 130 and 220 GHz. Those six CMB channels yield an aggregated CMB sensitivity of $2\,\mu$K arcmin 
($1.7\,\mu$K arcmin for the full array).
}
\label{tab:CORE-bands}
\end{table}
}


